A Benchmark and Dataset for Post-OCR text correction in Sanskrit

Sanskrit is a classical language with about 30 million extant manuscripts fit for digitisation, available in written, printed or scannedimage forms. However, it is still considered to be a low-resource language when it comes to available digital resources. In this work, we release a post-OCR text correction dataset containing around 218,000 sentences, with 1.5 million words, from 30 different books. Texts in Sanskrit are known to be diverse in terms of their linguistic and stylistic usage since Sanskrit was the 'lingua franca' for discourse in the Indian subcontinent for about 3 millennia. Keeping this in mind, we release a multi-domain dataset, from areas as diverse as astronomy, medicine and mathematics, with some of them as old as 18 centuries. Further, we release multiple strong baselines as benchmarks for the task, based on pre-trained Seq2Seq language models. We find that our best-performing model, consisting of byte level tokenization in conjunction with phonetic encoding (Byt5+SLP1), yields a 23% point increase over the OCR output in terms of word and character error rates. Moreover, we perform extensive experiments in evaluating these models on their performance and analyse common causes of mispredictions both at the graphemic and lexical levels. Our code and dataset is publicly available at https://github.com/ayushbits/pe-ocr-sanskrit.

==> relatedWork.tex <==
\section{Related Work}
OCR post-correction, a variant of grammatical error correction, has been extensively studied in the past.  However, such approaches are often ineffectual for morphologically rich languages, like ours, due to lexicon coverage issues.


%for high resource languages such as English. Early methods rely on  dictionary t. However, these methods do not reliably work for agglutinative or fusional languages due to high rate of out-of-vocabulary words. 

Recently, recurrent networks such as Recurrent Neural Networks or Long Short Term Memory (LSTM) networks have shown improved performance in Indic languages \cite{saluja2017error,saluja2019sub} due to their ability to remember longer context. \citet{krishna2018upcycle} used a neural seq2seq model meant for machine translation and added a a copy mechanism for enhanced performance on Romanized Sanskrit OCR. It generated synthetic images  and used it as a train set while test set consists of 430 real images. However, copying mechanism has not performed well within our setting.

Post-OCR correction methods on endangered languages by \citet{rijhwani2020ocr} proposed a multi-source architecture that leverages an initial OCR output and corresponding translation in a closely-related language using an attention mechanism. \citet{rijhwani2021lexically} used a semi-supervised approach that combines self-training with lexically-aware decoding on endangered languages. Prior works on Sanskrit \cite{saluja2017error} used LSTM-based methods on a small dataset of 86k words while our dataset consists of around 1.5 million words.

